Object classification on video data of meteors and meteor-like phenomena: algorithm and data

Every moment, countless meteoroids enter our atmosphere unseen. The detection and measurement of meteors offer the unique opportunity to gain insights into the composition of our solar systems' celestial bodies. Researchers, therefore, carry out a wide-area-sky-monitoring to secure 360-degree video material, saving every single entry of a meteor. Existing machine intelligence cannot accurately recognize events of meteors intersecting the earth's atmosphere due to a lack of high-quality training data publicly available. This work presents four reusable open source solutions for researchers trained on data we collected due to the lack of available labeled high-quality training data. We refer to the proposed dataset as the NightSkyUCP dataset, consisting of a balanced set of 10,000 meteor- and 10,000 non-meteor-events. Our solutions apply various machine learning techniques, namely classification, feature learning, anomaly detection, and extrapolation. For the classification task, a mean accuracy of 99.1\% is achieved. The code and data are made public at figshare with DOI: 10.6084/m9.figshare.16451625

==> content/hyperparameters.tex <==
\section{Hyperparameters of the classification experiments}\label{app:hyper}
We performed a hyperparameter optimization to find the best parameters for training, utilizing Nevergrad \cite{Rapin2018}, a Python library for gradient-free optimization. We used NGOpt8 as an optimizer.
The dataset used for optimization consists of $1000$ data points for each class. Our optimizations results are displayed in table \ref{tab:optimalParam}.
Data fusion was performed because we input both the image stacks and the stacks of metadata. 
We analysed the use of the fusion methods \textit{Late Feature Fusion} and \textit{Early Feature Fusion} (see figure \ref{fig:FusionTypes}).
We observed that for LSTM (Long short-term memory) and GRU (gated recurrent unit), the method of Early Feature Fusion is better, while for TCN (Temporal Convolutional Network), TDNN (Time Delay Neural Network), and AEC (Autoencoder), the Late Feature Fusion should be used.
\begin{table}[h!]
	\centering
	\begin{tabular}{|l||l|l|l|l|l|l|}
		\hline
		\textbf{} & \multicolumn{6}{c|}{\textbf{Optimal Parameters}} \\ \hline
		\textbf{Method} & \textbf{batch} & \textbf{lr} & \textbf{hidden} & \textbf{\# layer} & \textbf{context} & \textbf{kernel} \\ \hhline{|=#=|=|=|=|=|=|}
		LSTM & 16 & 0.001 & 900 & 1 & \cellcolor{lightgray!50} & \cellcolor{lightgray!50} \\ \hline
		GRU & 16 & 0.001 & 250 & 1 & \cellcolor{lightgray!50} & \cellcolor{lightgray!50} \\ \hline
		TDNN Feature & 16 & 0.001 & 30 & \cellcolor{lightgray!50} & 10 & \cellcolor{lightgray!50} \\ \hline
		TDNN Meta & 8 & 0.01 & 120 & \cellcolor{lightgray!50} & 8 & \cellcolor{lightgray!50} \\ \hline
		TDNN Classifier & 8 & 0.01 & \cellcolor{lightgray!50} & \cellcolor{lightgray!50} & \cellcolor{lightgray!50} & \cellcolor{lightgray!50} \\ \hline
		TCN Feature & 16 & 0.0001 & 10 & 7 & \cellcolor{lightgray!50} & 2 \\ \hline
		TCN Meta & 64 & 0.01 & 20 & 3 & \cellcolor{lightgray!50} & 50 \\ \hline
		TCN Classifier & 8 & 0.001 & \cellcolor{lightgray!50} & \cellcolor{lightgray!50} & \cellcolor{lightgray!50} & \cellcolor{lightgray!50} \\ \hline
		AEC Feature & 8 & 0.001 & 60 & \cellcolor{lightgray!50} & \cellcolor{lightgray!50} & \cellcolor{lightgray!50} \\ \hline
		AEC Meta & 16 & 0.0001 & 400 & \cellcolor{lightgray!50} & \cellcolor{lightgray!50} & \cellcolor{lightgray!50} \\ \hline
		AEC Classifier & 8 & 0.001 & \cellcolor{lightgray!50} & \cellcolor{lightgray!50} & \cellcolor{lightgray!50} & \cellcolor{lightgray!50} \\ \hline
	\end{tabular}
	\caption{Results of the hyperparameter optimization. For methods trained with \textit{Late Feature Fusion} (LFF), the individual networks must be optimized separately for the metadata and the feature data. Furthermore, learning rate and batch size are determined for the joint classifier, a single fc-layer. The batch size is described by \textit{batch}, \textit{hidden} and \textit{kernel} represent the number of neurons in the hidden layer and the size of the kernels. \textit{lr} represents the learning rate. Since not every method has the same hyperparameters, the cells of unassociated parameters are grayed out.}
	\label{tab:optimalParam}
\end{table}
\begin{figure}[h!]
	\centering
	\begin{subfigure}[b]{0.8\textwidth}
		\centering
		\includegraphics[width=\textwidth]{Fusion_Type1}
		\caption{Early Feature Fusion}
		%\label{fig:y equals x}
		\vspace*{2em}
	\end{subfigure}
	\begin{subfigure}[b]{0.8\textwidth}
		\centering
		\includegraphics[width=\textwidth]{Fusion_Type2}
		\caption{Late Feature Fusion}
		%\label{fig:three sin x}
	\end{subfigure}
	\caption{Representation of the examined fusion types. The blocks \textit{NN (Neuronal Network)} are representative of the different feature extraction methods which are investigated. For the fusion of the data, represented by $\otimes$, concatenation was used.}
	\label{fig:FusionTypes}
\end{figure}
